Large Scale GAN Training for High Fidelity Natural Image Synthesis

Despite recent progress in generative image modeling, successfully generating high-resolution, diverse samples from complex datasets such as ImageNet remains an elusive goal. To this end, we train Generative Adversarial Networks at the largest scale yet attempted, and study the instabilities specific to such scale. We find that applying orthogonal regularization to the generator renders it amenable to a simple "truncation trick," allowing fine control over the trade-off between sample fidelity and variety by reducing the variance of the Generator's input. Our modifications lead to models which set the new state of the art in class-conditional image synthesis. When trained on ImageNet at 128x128 resolution, our models (BigGANs) achieve an Inception Score (IS) of 166.5 and Frechet Inception Distance (FID) of 7.4, improving over the previous best IS of 52.52 and FID of 18.6.

==> BigGAN arXiv/ablation_table.tex <==
\begin{table}[tbp]
\small
\begin{center}\begin{tabular}{c|c|c|c|c|c|c|c|c} 
\hline
 Batch & Ch. & Param (M)  & Shared & Skip-$z$ & Ortho. & Itr $\times 10^3$ & FID  & IS \\

\hline   256& 64 & 81.5  &\multicolumn{3}{c|}{SA-GAN Baseline} & $1000$ &  $18.65$  & $ 52.52 $\\ % Baseline, params:  G: 42017412, D: 39448258, total 81465670
\hline   512 & 64 & 81.5  & \xmark & \xmark & \xmark & $1000$ &  $15.30$  & $58.77 (\pm 1.18) $\\ % setting 1, params:  G: 42017412, D: 39448258, total 81465670

\hline   1024 & 64 & 81.5  & \xmark & \xmark &\xmark & $1000$ &  $14.88$ & $63.03 (\pm 1.42)$\\ % setting 2, params: G: 42017412, D: 39448258, total 81465670

\hline   2048 & 64 & 81.5  & \xmark & \xmark &\xmark & $732$ &  $12.39$ & $76.85 (\pm 3.83)$\\ % setting 3, params: G: 42017412, D: 39448258, total 81465670
  
\hline   2048 & 96 & 173.5  & \xmark & \xmark &\xmark & $295 (\pm 18)$ &  $9.54 (\pm 0.62)$ & $92.98 (\pm 4.27)$\\ % setting 2.1, params: G: 85556164, D: 87982370, total 173538534

\hline   2048 & 96 & 160.6  & \cmark & \xmark &\xmark & $185 (\pm 11) $ &  $9.18 (\pm 0.13)$ & $94.94 (\pm 1.32)$\\ % setting 2.2, params:  G: 72664516, D: 87982370, total 160646886

\hline   2048 & 96 & 158.3  & \cmark & \cmark &\xmark & $152 (\pm 7)$ & $8.73 (\pm 0.45)$ & $98.76 (\pm 2.84)$\\ % setting 2.3, params: G: 70305988, D: 87982370, total 158288358

\hline   2048 & 96 & 158.3  & \cmark & \cmark &\cmark & $165 (\pm 13)$ &  $8.51 (\pm 0.32)$ & $99.31 (\pm 2.10)$\\ %  setting 2.4, params: G: 70305988, D: 87982370, total 158288358

\hline   2048 & 64 & 71.3  & \cmark & \cmark &\cmark & $371 (\pm 7) $ &  $10.48 (\pm 0.10) $ & $ 86.90 (\pm 0.61)$\\ % setting 2.7, params: G: 31850628, D: 39448258, total 71298886

\hline

\end{tabular}
\end{center}

\caption{\label{ablation_table} Fr\'echet Inception Distance (FID, lower is better) and Inception Score (IS, higher is better) for ablations of our proposed modifications. \textit{Batch} is batch size, \textit{Param} is total number of parameters, \textit{Ch.} is the channel multiplier representing the number of units in each layer, \textit{Shared} is using shared embeddings, 
% \textit{Skip-$z$} is using a hierarchical latent space,
\textit{Skip-$z$} is using skip connections from the latent to multiple layers, 
\textit{Ortho.} is Orthogonal Regularization, and \textit{Itr} indicates if the setting is stable to $10^6$ iterations, or it collapses at the given iteration. Other than rows 1-4, results are computed across 8 random initializations.
}
\end{table}

==> BigGAN arXiv/jft_table.tex <==
\begin{table}[tbp]
\small
\begin{center}\begin{tabular}{c|c|c|c|c|c|c|c|c} 
\hline
 %Res. & Batch & Ch. & Param (M) & Shared & Hier. & Ortho. & FID & IS \\
 Ch. & Param (M) & Shared & Skip-$z$ & Ortho. & FID & IS & (min FID) / IS & FID / (max IS) \\
\hline
%\multirow{4}{*}{256}
% G: 254953092, D: 62152898 = 317,105,990
 64 & 317.1 & \xmark & \xmark & \xmark & $48.38$ & $23.27$ & $48.6 / 23.1$ & $49.1 / 23.9$ \\
\hline
% G: 37197444, D: 62152898 = 99,350,342
 64 & 99.4 & \cmark & \cmark & \cmark & $23.48$ & $24.78$ & $22.4 / 21.0$ & $60.9 / 35.8$ \\
\hline
% G: 82107844, D: 125786402 = 207,894,246
 96 & 207.9 & \cmark & \cmark & \cmark & $18.84$ & $27.86$ & $17.1 / 23.3$ & $51.6 / 38.1$ \\
\hline
% G: 144559364, D: 211124610 = 355,683,974
128 & 355.7 & \cmark & \cmark & \cmark & $13.75$ & $30.61$ & $13.0 / 28.0$ & $46.2 / 47.8$ \\
\hline
\end{tabular}
\end{center}
\caption{
\label{jft_table}
%Results on the internal dataset at $256\times256$ resolution.
%The \textit{FID} and \textit{IS} columns report these scores given by the internal dataset-trained Inception v2 classifier with noise distributed as $z \sim \mathcal{N}(0, I)$ (non-truncated).
%The \textit{(min FID) / IS} and \textit{FID / (max IS)} columns report scores at the best FID and IS from a sweep across truncated noise distributions ranging from $\sigma = 0$ to $\sigma = 2$.
%Images from the validation set have an IS of 50.88 and FID of 1.94.
BigGAN results on JFT-300M at $256\times256$ resolution.
The \textit{FID} and \textit{IS} columns report these scores given by the JFT-300M-trained Inception v2 classifier with noise distributed as $z \sim \mathcal{N}(0, I)$ (non-truncated).
The \textit{(min FID) / IS} and \textit{FID / (max IS)} columns report scores at the best FID and IS from a sweep across truncated noise distributions ranging from $\sigma = 0$ to $\sigma = 2$.
Images from the JFT-300M validation set have an IS of 50.88 and FID of 1.94.
}
\end{table}


% train+val set:
% (JFT) inception_score = 50.659447,+/- 1.394818, acc: -1.000000, FID = 1.914317  duration = 139.051551 s
% 
% test set:
% (JFT) inception_score = 50.883789,+/- 4.031054, acc: -1.000000, FID = 1.935230  duration = 139.914789 s

==> BigGAN arXiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> BigGAN arXiv/results_table.tex <==
% Results table for Experiments section
% Note that for FIDs we might just report e.g. "6.34 (\pm .21)" instead of (\pm0.21) to save space (can't fit that tasty leading zero =(
\begin{table}[tbp]
\small
\begin{center}\begin{tabular}{c|c|c|c|c|c} 
\hline
Model & Res. &    FID/IS   & (min FID) / IS & FID / (valid IS) & FID / (max IS) \\

\hline \hline
SN-GAN & 128 & $27.62 / 36.80$ & N/A & N/A & N/A \\

\hline 
SA-GAN & 128 & $18.65 / 52.52$ & N/A & N/A & N/A \\

\hline\hline
BigGAN & 128 & $8.7\pm.6/98.8\pm3$ & $7.7\pm.2/126.5\pm 0$  & $9.6\pm.4/166.3\pm1$ & $25\pm2/206\pm2$ \\

\hline 
BigGAN & 256 & $8.7\pm.1/142.3\pm2$ & $7.7\pm.1/178.0\pm5$ & $9.3\pm.3/233.1\pm1$ & $25\pm5/291\pm4$ \\

\hline 
BigGAN & 512 & $8.1 / 144.2$  & $7.6 / 170.3$  & $11.8 / 241.4$ & $27.0 / 275$ \\

\hline \hline
BigGAN-deep & 128 & $5.7 \pm .3/124.5 \pm 2$ & $6.3 \pm .3/148.1 \pm 4$  & $7.4 \pm .6/166.5 \pm 1$ & $25 \pm 2/253 \pm 11$ \\

\hline
BigGAN-deep & 256 & $6.9 \pm .2/171.4 \pm 2$ & $7.0 \pm .1/202.6 \pm 2$ & $8.1 \pm .1/232.5 \pm 2$ & $27 \pm 8/317 \pm 6$ \\

\hline
BigGAN-deep & 512 & $7.5/152.8$  & $7.7/181.4$  & $11.5/241.5$ & $39.7/298$ \\

\hline
\end{tabular}
\end{center}

\caption{\label{results_table} Evaluation of models at different resolutions. We report scores without truncation (Column 3), scores at the best FID (Column 4), scores at the IS of validation data (Column 5), and scores at the max IS (Column 6). Standard deviations are computed over at least three random initializations.}
\end{table}

==> BigGAN arXiv/results_table_overfull.tex <==
% Results table for Experiments section
% Note that for FIDs we might just report e.g. "6.34 (\pm .21)" instead of (\pm0.21) to save space (can't fit that tasty leading zero =(
\begin{table}[tbp]
\small
\begin{center}\begin{tabular}{c|c|c|c|c|c} 
\hline
        Model & Res. &    FID/IS   & (min FID) / IS & FID / (valid IS) & FID / (max IS) \\
        % Model &     Resolution &    FID/IS   & FID/ISv1 & FID/ISv2  \\

\hline SN-GAN & 128 & 27.62 / 36.80 & N/A & N/A & N/A \\

\hline SA-GAN & 128 & 18.65 / 52.52 & N/A & N/A & N/A \\

%IS of valid data at 128x128 is 165.126312 +/- 8.106392

% Iterations over rounding to make this table fit
% \hline BigGAN & 128$\times$128 & $8.73 (\pm .45)$/$98.76 (\pm 2.84)$ & $7.74 (\pm .04)$ / $126.51 (\pm .04)$  & $9.57 (\pm .39)$/$166.34 (\pm .68)$  & values\\
% \hline BigGAN & 128 & $8.73$ / $98.76$ & $7.74$ / $126.51$  & $9.57$ / $166.34$ & N/A \\
% \hline BigGAN & 128$\times$128 & $8.73\pm.55$/$98.8\pm2.8$ & $7.74\pm.04$/$126.5\pm.04$  & $9.57\pm.4$/$166.3\pm .7$ & values  \\
\hline BigGAN & 128 & $8.7\pm.6$/$98.8\pm2.8$ & $7.7\pm.1$/$126.5\pm.1$  & $9.6\pm.4$/$166.3\pm1$ & $25\pm2/206\pm2$ \\



% IS of valid data at 256x256 is 230.667938 +/- 10.150323
% These numbers here are for a single run, not averaged
% \hline BigGAN & 256 & $8.40 $ / $150.34$  & $7.65$ / $184.30$  & $9.26$ / $231.86$ & values \\
\hline BigGAN & 256 & $8.2\pm.2$/$154\pm2.5$ & $7.7\pm.1$/$178\pm5$ & $9.3\pm.3$/$233\pm1$ & $25\pm5$/$295\pm4$ \\
% \hline BigGAN & 256$\times$256 & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  \\

% IS of valid data for IHQ400 is 240.021454 +/- 15.395828
% \hline BigGAN & 512 & $10.86$ / $154.876$  & $9.34$ / $202.5$  & $10.88$ / $241.36$ & values \\
\hline BigGAN & 512 & $10.9$ / $154.9$  & $9.3$ / $202.5$  & $10.9$ / $241.4$ & $24.4$/$275$ \\
% \hline BigGAN & 512$\times$512 & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  \\

\hline
\end{tabular}
\end{center}

\caption{\label{results_table} Evaluation of models at different resolutions. We report scores without truncation (Column 3), scores at the best FID (Column 4), scores at the IS of validation data (Column 5), and scores at the max IS (Column 6). Standard deviations are computed over at least three random initializations.}
\end{table}

==> results_table_overfull.tex <==
% Results table for Experiments section
% Note that for FIDs we might just report e.g. "6.34 (\pm .21)" instead of (\pm0.21) to save space (can't fit that tasty leading zero =(
\begin{table}[tbp]
\small
\begin{center}\begin{tabular}{c|c|c|c|c|c} 
\hline
        Model & Res. &    FID/IS   & (min FID) / IS & FID / (valid IS) & FID / (max IS) \\
        % Model &     Resolution &    FID/IS   & FID/ISv1 & FID/ISv2  \\

\hline SN-GAN & 128 & 27.62 / 36.80 & N/A & N/A & N/A \\

\hline SA-GAN & 128 & 18.65 / 52.52 & N/A & N/A & N/A \\

%IS of valid data at 128x128 is 165.126312 +/- 8.106392

% Iterations over rounding to make this table fit
% \hline BigGAN & 128$\times$128 & $8.73 (\pm .45)$/$98.76 (\pm 2.84)$ & $7.74 (\pm .04)$ / $126.51 (\pm .04)$  & $9.57 (\pm .39)$/$166.34 (\pm .68)$  & values\\
% \hline BigGAN & 128 & $8.73$ / $98.76$ & $7.74$ / $126.51$  & $9.57$ / $166.34$ & N/A \\
% \hline BigGAN & 128$\times$128 & $8.73\pm.55$/$98.8\pm2.8$ & $7.74\pm.04$/$126.5\pm.04$  & $9.57\pm.4$/$166.3\pm .7$ & values  \\
\hline BigGAN & 128 & $8.7\pm.6$/$98.8\pm2.8$ & $7.7\pm.1$/$126.5\pm.1$  & $9.6\pm.4$/$166.3\pm1$ & $25\pm2/206\pm2$ \\



% IS of valid data at 256x256 is 230.667938 +/- 10.150323
% These numbers here are for a single run, not averaged
% \hline BigGAN & 256 & $8.40 $ / $150.34$  & $7.65$ / $184.30$  & $9.26$ / $231.86$ & values \\
\hline BigGAN & 256 & $8.2\pm.2$/$154\pm2.5$ & $7.7\pm.1$/$178\pm5$ & $9.3\pm.3$/$233\pm1$ & $25\pm5$/$295\pm4$ \\
% \hline BigGAN & 256$\times$256 & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  \\

% IS of valid data for IHQ400 is 240.021454 +/- 15.395828
% \hline BigGAN & 512 & $10.86$ / $154.876$  & $9.34$ / $202.5$  & $10.88$ / $241.36$ & values \\
\hline BigGAN & 512 & $10.9$ / $154.9$  & $9.3$ / $202.5$  & $10.9$ / $241.4$ & $24.4$/$275$ \\
% \hline BigGAN & 512$\times$512 & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  & $0.0 (\pm 0.0)$/$0.0 (\pm 0.0)$  \\

\hline
\end{tabular}
\end{center}

\caption{\label{results_table} Evaluation of models at different resolutions. We report scores without truncation (Column 3), scores at the best FID (Column 4), scores at the IS of validation data (Column 5), and scores at the max IS (Column 6). Standard deviations are computed over at least three random initializations.}
\end{table}
